Cybersecurity in Robotics: Challenges, Quantitative Modeling, and Practice

Robotics is becoming more and more ubiquitous, but the pressure to bring systems to market occasionally goes at the cost of neglecting security mechanisms during the development, deployment or while in production. As a result, contemporary robotic systems are vulnerable to diverse attack patterns, and an a posteriori hardening is at least challenging, if not impossible at all. This book aims to stipulate the inclusion of security in robotics from the earliest design phases onward and with a special focus on the cost-benefit tradeoff that can otherwise be an inhibitor for the fast development of affordable systems. We advocate quantitative methods of security management and design, covering vulnerability scoring systems tailored to robotic systems, and accounting for the highly distributed nature of robots as an interplay of potentially very many components. A powerful quantitative approach to model-based security is offered by game theory, providing a rich spectrum of techniques to optimize security against various kinds of attacks. Such a multi-perspective view on security is necessary to address the heterogeneity and complexity of robotic systems. This book is intended as an accessible starter for the theoretician and practitioner working in the field.

==> ArXiv Version Robot Security Updated V4/subsections/control.tex <==
\subsection{Resilient Control Mechanisms and Real-Time System Performance}

In Section \ref{msmp}, we have used a multi-stage and multi-phase game to capture how an attacker moves from the cyber layer to the physical layer. The physical layer of robotics consists of the real-time dynamics represented by the system model in (\ref{dynamics}). It also corresponds to level $0$ of the ROS architecture, illustrated in Fig. \ref{fig:networking_multi_agent_architecture}. The defense at the physical layer heavily relies on the resilient control mechanisms when the attacker has successfully taken control of the devices at the field network. The purpose of resilient control is to enable the robotic systems to maintain a satisfactory level of performance when the robotic system is attacked by unanticipated threats in real-time. An example of such resilient control mechanisms is introduced in \citep{xu2015secure} for cloud robotics. A UAV that relies on the cloud for communication and information processing can switch from an optimal mode of operations to a safe mode when a man-in-the-middle attack is detected. 

As discussed in \citep{zhuchapter}, resilient control is divided into three stages: ex-ante planning, interim execution, and ex-post recovery. The ex-ante stage is the resilience planning that designs contingency plans to prepare for the anticipated attacks. The interim execution stage is the operation stage of the control system, which executes the resilience plans in real-time. A resilient operation includes online learning for anomaly detection and adaptive decision-making for responding to the anomaly. The ex-post recovery refers to the recovery process in which the robots can still maintain critical functions or heal themselves to complete the tasks.

The three-stage resilient control mechanism is the last resort to safeguard the robotic systems and mitigate the impact of physical damages. This approach is complementary to the cyber defense designed at the penultimate level to prevent an attacker to reach the final level. Perfect security is not practicable in real-time systems as it would significantly increase the cost and reduce the usability of cybersecurity and resilient control mechanisms can be designed jointly to effectively reduce the impact of cyber threats. The cyber defense in the joint design needs to anticipate the consequence when the attacker successfully evades the defense and reaches the physical asset. Meanwhile, the design of a resilient control mechanism needs to take into account the effectiveness of the cyber defense and design resiliency in response to possible successful attacks.
This joint design methodology aligns with the games-in-games defense paradigm introduced in Section \ref{gigm}. The resilient control is subsumed in the last stage design, or G3 in Fig. \ref{nestedgames}, while the cyber defense is viewed as the outcome of G1 and G2. In \citep{zhu2012dynamic,zhu2011robust}, resilient control is viewed as a game between the controller and the worst-case scenario that can occur to the real-time system. Therefore, the games-in-games design paradigm provides a holistic view to understand the impact of cyber defense on the real-time system performance and design cross-layer defense and resilient control mechanisms.


%It enables the design defenses at earlier stages that optimize its performance requirements by reducing the success rate of an attack.




==> ArXiv Version Robot Security Updated V4/subsections/quanyan-game.tex <==
\section{Introduction to Security Games and Strategic Defenses}\label{gamemodels}

We have seen in recent years that attackers are becoming increasingly sophisticated and intelligent. Traditional security solutions that rely on cryptography, firewalls, and intrusion detection systems are \emph{necessary} (cf. Section \ref{sec:securing-the-api}) but not \emph{sufficient} to guarantee the security of the robots. There are many ways that an attacker can circumvent these technologies and gain access to the targeted systems. The design objective of perfect security is not possible as the system designers are always constrained by resources. The attack graph from Section \ref{sec:cut-the-rope} is one step towards this: instead of aiming for perfect security, one reasonable security solution is to understand the specific system features and their objectives and take into account the strategic behaviors of the attacks and the constraints on the attack-and-defense resources. In robotic systems, the consequences of a compromised system differ depending on the domain of the applications. For example, a service robot that interacts with humans, e.g., self-driving cars and autonomous vehicles, can be turned into a deadly weapon that hurts human users. Manufacturing robots on assembly lines can break down and cause a significant economic loss due to reduced production. Hence understanding and quantifying the system-specific objectives and the available resource is key to developing an effective defense mechanism against attackers.
%There is a need of a new security paradigm where security solutions take intou account t The consequence is significant.

To this end, game theory provides a modeling and reasoning framework for the design of effective security solutions \citep{manshaei2013game}. First, game-theoretic models can capture the competitive and strategic behaviors of the players and their constraints. Second, there are a rich set of game-theoretic algorithms and tools that enable the prediction of the outcomes through the analysis and the computation of the equilibrium. Third, game models provide ways to incorporate human factors, including bounded rationality, cognitive biases, and human perception. Fourth, game models can take different forms at multiple layers of the system and for various attack models. They can be composed and integrated to create a game of games to provide a holistic view of the security issues across the layers of the system and enable a design of system-wide security solutions. Game theory has been used in a wide variety of cybersecurity contexts. A few application areas include intrusion detection systems \citep{zhu2011indices,zhu2010network,zhu2009dynamic}, adversarial machine learning \citep{zhang2015secure,pawlick_stackelberg_2016,zhang2016dynamic,zhang_game-theoretic_2017,zhang2018gameML}, proactive and adaptive defense \citep{van2013flipit,farhang2014dynamic,clark2012deceptive,zhu2011distributed,zhu2010heterogeneous,zhu2010no,huang2010distributed}, cyber deception \citep{zhu2012dynamic,zhang2019game,Huang2019,pawlick2018modeling,Pawlick2018Dissertation,pawlick2017game},  communications channel jamming \citep{basar1983gaussian,zhu2011eavesdropping,zhu2010stochastic,xu_game-theoretic_2017,zhu2011dynamic,zhu2013game}, secure industrial control systems \citep{miao2014moving,zhu2015game,zhu2012dynamic,alpcan2004game} and critical infrastructure security and resilience \citep{rass_gadapt:_2016,chen_interdependent_2016-1,huang2019adaptive,chen_interdependent_2016,huang2018analysis,huang2017large,huang2018distributed}.

\subsection{Models and Security Games}\label{sec:game-theory-definitions}

Let us reconsider the intuitive description of games laid out in Section \ref{sec:game-theory-intro}, in more rigorous and general terms: 
A normal form game of complete information is defined by three elements. The
first one is the set of players, denoted by $\mathcal{N}$. In security games,
there are often two players in the game. One is the attacker $A$. The other
one is the defender $D$. The second element is the action set of the players,
denoted by $\mathcal{A}_i, i\in\mathcal{N}$. The action set captures the
feasible actions that are available to the players. It can naturally
incorporate the system and knowledge constraints of the players, and the
rules of the games. The third element is the preference or the payoffs of the
players $U_i, i\in \mathcal{N}$, which depends on the actions played by all
players, $\{a_i, i\in\mathcal{N}\}$, known as the action profile. Each player
chooses to play the action that maximizes his payoff. We are interested in
the outcome of this game when the players have complete information of this
game and choose action $a_i \in \mathcal{A}_i$ to maximize their own payoff.
The normal-form game of two players with finite actions, say the row player
$A$ and the column player $D$, can be represented by a matrix. Each row $k
\in\{1, 2, \ldots, n\}$ corresponds to an action in the action set of player
$A$; each column $l \in \{1, 2, \ldots, m\}$ corresponds to an action in the
action set of player $D$. Matrices $F, G \in \mathds{R}^{n\times m}$ are the
payoff matrices for players $A, D$, respectively. Entries $F_{kl}, G_{kl}$
represent the payoff to players $A, D$, respectively, when actions that
correspond to $k$-th row and $l$-th column are played.

This outcome is predicted by the solution concept called Nash equilibrium. An action profile $\{a_i^*\in\mathcal{A}_i, i\in\mathcal{N}\}$ constitutes a (pure-strategy) Nash equilibrium when no player can deviate from it unilaterally; in other words,
$$
U_i(a^*_i, a^*_{-i}) \geq U_i(a_i, a^*_{-i}),
$$
 for all $a_i\in \mathcal{A}_i, i\in\mathcal{N}$. Here, $a^*_{-i}$ is the set of all equilibrium actions $\{a^*_i, i\in\mathcal{N}\}$ excluding the equilibrium action of player $i$, i.e., $a_i^*$. The Nash equilibrium of an $N$-person game defined by the triplet $\left(\mathcal{N}, \{\mathcal{A}_i\}_ {i\in\mathcal{N}}, \{U_i\}_ {i\in\mathcal{N}} \right)$ may not  exist. However, the existence issue is resolved when we extend the strategy space to mixed strategies, which are essentially \emph{probability distributions} over the action spaces that describe \emph{random choice rules} for taking actions in the game: Let $x_i, i\in\mathcal{N},$ be the mixed strategies of player $i$. Its $j$-th component $x_i(a_j)$ can be interpreted as the probability of player $i$ choosing action $a_j$ from the discrete action set $\mathcal{A}_i$. It is clear that $x_i(a_j)$ is nonnegative and $\sum_{a_j\in\mathcal{A}_i} x_i(a_j) =1$. Under the mixed strategy profile $\{x_i, i\in\mathcal{N}\}$, the payoff received by the player is the average payoff $\bar{U}_i(x_i, x_{-i})$, which is merely a weighted sum using the payoffs from the actions, multiplied with their corresponding probabilities from the mixed strategy. In the case of two-player games, let $x_1, x_2$ be the mixed strategies represented as a finite-dimensional vectors (of appropriate dimension) of the row player and the column player, respectively. The $k$-th component of $x_1$ and the $l$-th component of $x_2$ correspond to the probabilities of the row player (resp. column player) choosing actions associated with $k$-th row (resp. $l$-th column). The average payoff to the row player is given by $\bar{U}_1=x_1^TFx_2$; the average payoff to the column player is given by  $\bar{U}_2=x_1^TGx_2$.


 The mixed-strategy Nash equilibrium can be defined in a similar way as the pure-strategy Nash equilibrium. The mixed-strategy profile $\{x_i^*, i\in\mathcal{N}\}$ constitutes a mixed-strategy Nash equilibrium if for all admissible mixed strategy $x_i, i\in\mathcal{N}$,
$$
\bar{U}_i(x^*_i, x^*_{-i}) \geq \bar{U}_i(x_i, x^*_{-i}).
$$
It has been known that there exists a mixed-strategy Nash equilibrium for every finite normal-form game \citep{basar1999dynamic,nash1950equilibrium}.

Zero-sum games are a special class of games that are often used to model strictly competitive behaviors between two players. One player's gain is the other player's loss. In other words, let $U_1(a_1, a_2)=-U_2(a_1, a_2)= U(a_1, a_2)$. Player 1's objective is to maximize the payoff $U$ while Player 2's objective is to minimize it. The roles of who maximizes and who minimizes can, however, be freely exchanged, and the game \textsc{Cut-The-Rope} is an example where the defender is a minimizer: indeed, the defender's payoff in Section \ref{sec:cut-the-rope} is simply the probability for the attacker to hit the vital target asset, which naturally should be small if the defense is good. In turn, the attacker obviously seeks to maximize this probability, and we have a zero-sum competition here. 

  The solution concept of zero-sum games is \emph{saddle-point equilibrium}: this is a joint strategy $(a_1^*, a_2^*)$ if for all $a_1\in\mathcal{A}_1$ and $a_2\in\mathcal{A}_2$,
$U(a_1, a_2^*) \leq U(a_1^*, a_2^*) \leq U(a_1^*, a_2)$, and called \emph{pure} if the strategies $a_1^*, a_2^*$ are pure. A two-person zero-sum game can be represented by one matrix $H$.  Row $i$ of the matrix corresponds to the $i$-th action of the row player, say the defender. Column $j$ of the matrix corresponds to the $j$-th action of the column player, say the attacker. The entry of the matrix $H_{ij}$ is the payoff to the defender, i.e., the loss to the attacker when the defender plays the $i$-th action and the attacker plays the $j$-th action. Let $x_1$ and $x_2$ be the mixed strategies of the players. The average payoff or loss to player 1 or player 2, respectively, is given by
$\bar{U}(x_1, x_2) = x_1^THx_2$. Here, $x_1, x_2$, and $H$ are vectors and matrix of appropriate dimensions.  A mixed strategy $(x_1^*, x_2^*)$ is a mixed-strategy saddle-point equilibrium if for all admissible $x_1, x_2$,
$\bar{U}(x_1, x_2^*) \leq \bar{U}(x_1^*, x_2^*) \leq \bar{U}(x_1^*, x_2)$.   The value $\bar{U}$ achieved under the equilibrium profile is called the \emph{value} of the game. 

Returning to \textsc{Cut-The-Rope} (Section \ref{sec:cut-the-rope}) again for illustration, the value would be the last number $v=0.001$ in \eqref{eqn:cut-the-rope-example-equilibrium}, since the game is primarily about minimizing the attacker's chances to hit its target. Any deviation towards a different defense than prescribed by the game would just increase the success chances for the adversary to more than $0.001$. This is important for the defender to bear in mind, since an attempt to further decrease the protection in other places may open the door wider for the attacker: for example, if the defender is okay with the probability of $0.001$ for the attacker to hit node 10, but then strives to decrease the -- seemingly high -- probability of $0.228$ for the attacker to be at node 9 instead, any change in the defense strategy for the sake of lowering the number $0.228$ would imply an increase of the attacker's chance to hit node 10 perhaps on other ways, say, bypassing node 9 at all! This effect is due to the equilibrium property formalized above.

One important property of saddle-point equilibrium is the exchangeability; i.e., when $(x_1^*, x_2^*)$ and $(x_1^\circ, x_2^\circ)$ are two distinct saddle-point equilibria of the zero-sum game, then $(x_1^*, x_2^\circ)$ and $(x_1^\circ, x_2^*)$ are also saddle-point equilibria of the game and yield the same game value. This is the theoretical reason why it is safe for the defender to use \emph{any} of the existing equilibria for its defensive purpose, but at the same time dangerous to rely on the adversary's equilibrium as a hint on where to defend: the exchangeability property lets the adversary pick any of (perhaps many) optimal attack strategies to gain the best possible success rates, which can easily annihilate the defender's precautions if they were based on the attacker's equilibrium behavior instead of the (better) defender's equilibrium strategies.

\subsection{Structural and Operational Security}\label{sec:example-games}

Zero-sum games are useful to capture many security scenarios. For example, a jamming game between a team of  {UAV} and a jammer has been investigated in \cite{chen-TCNS-19-games}. Illustrated in Fig. \ref{team}, a team of  {UAV} is controlled to maximize the connectivity among themselves in an adversarial environment where an attacker can choose a subset of communication links to jam. The game between the operator of the team and the attacker is described by the zero-sum game at time $k$:
\begin{equation}\label{maxminproblem}
 \max_{x(k+c)}\min_{e\in \mathcal{E}} \lambda_2(e; x(k + c)).
 \end{equation}
Here, $x(k)$ is the position of the  {UAV} at time $k$. Two  {UAV} can form a link when they are sufficiently close within
a desirable range of communications. The connectivity of the  {UAV} team is described by the algebraic connectivity of the network, denoted by $\lambda_2$ (i.e., the second-smallest eigenvalue of the associated Laplacian matrix). When $\lambda_2$ is zero, the network has disjoint partitions. Otherwise, the network is connected, i.e., there exists a path from one node to any node in the network. A higher value of $\lambda_2$ indicates that there are a larger number of paths on average that connect between two arbitrary nodes in this network.  At each time
step $k$, the operator determines where the agents should move to in the next time step
$x(k + c)$, where $c$ is a time interval. The control is constrained by the physical dynamics
of  {UAV}. The attacker can jam a subset of links from all the communication links of the team, denoted by $\mathcal{E}$. The attacker's capability is described by the number of links that he can jam at time $k$. This zero-sum security game can be played repeatedly at every time step $k$.

 \begin{figure}[t]
    \centering
     \includegraphics[scale=0.5]{figures/team.png}
    \caption{A team of  {UAV} collaborate on a mission. They can communication with each other when one is in the range of communication of the other. An attacker can jam the signals between two  {UAV}.} \label{team}
\end{figure}

In transportation networks, the class of interdiction games is similar to the jamming games in communications. One player (e.g., an attacker) aims to remove the links of a network to minimize the throughput or disrupt the operation of the infrastructure subject to resource constraints. In other words, the attacker's capability is assumed to be bounded and he can only remove a small subset of links in the network.  The other player (e.g., planner or defender) aims to design a robust network and invest resources to protect against the attacks on the network and maintain the service of the infrastructure.   This type of games has been commonly used in scenarios of the infrastructure protections \citep{chen2019dynamic,huang2017large,chen2019game}, multi-agent robotic systems \citep{nugraha2020dynamic,chen-CDC-16,chen-TCNS-19-games}, and  {IoT} networks \citep{chen2017heterogeneous,Chen2019optimal}.%and The analysis of the zero-sum game between the attacker and the defender enables the planner to find the optimal
%A generalized version of this has been studied in \cite{goyal,juntao}

Another example of security game is the system configuration game \citep{zhu2011indices,zhu2009dynamic,zhu2010network}. In this game, we consider one system defender and one attacker as two players. The system defender configures its network and  {IoT} in Fig. \ref{fig:cut-the-rope} %\stefan{@Quanyan: broken reference? Which picture do you mean here?} 
by choosing the setting of the software, security rules/policies, and network topologies. Each system configuration inevitably has known or zero-day vulnerabilities. An attacker aims to find the vulnerabilities of the entry-point system and exploit them to penetrate and infect further parts of the system. Let $\mathcal{C}= \{c_1, c_2, \cdots, c_m\} $ be the set of configuration that the system can choose from. Let $\mathcal{V}$ be the set of vulnerabilities that the system can have. Each configuration is associated with a subset of vulnerabilities of $\mathcal{V}$. We let $\pi: \mathcal{C}\rightarrow 2^\mathcal{V}$ be the point-to-set mapping between configurations and the subsets of vulnerabilities; $\pi(c),\subseteq \mathcal{V}, c\in \mathcal{C},$ is called the attack surface when the system is configured to $c$. An attacker can choose an attack that exploits several vulnerabilities of the system. Let $\mathcal{A}=\{a_1, a_2, \cdots, a_n\}$ be the set of attack actions. Let $\gamma: \mathcal{A}\rightarrow 2^\mathcal{V}$ be the point-to-set mapping between attack actions and the subset of vulnerabilities; $\gamma(a) \subseteq \mathcal{V}, a\in\mathcal{A},$ is the set of vulnerabilities exploited by the attack action $a\in\mathcal{A}$. When one of the vulnerabilities exploited by the attacker is in the attack surface under configuration $c$, then the attacker is successful and receives a reward. More formally, when $\gamma(a) \cap \pi(c) \neq \emptyset$, the reward to the attacker, which is also the loss to the defender, is given by $R(\gamma(a) \cap \pi(c))$, where $R$ is a set-valued function that quantifies the impact of the successfully exploited vulnerabilities. This configuration game is a normal-form zero-sum game. An example of this game is represented by the following matrix:

\begin{center}
{H:}
  \begin{tabular}{ l | c | c | c | c }
     & $c_1$ & $c_2$ & $c_3$ & $c_3$ \\ \hline
    $a_1$ & $h_{11}$ & $h_{12}$ & $ h_{13}$ & $h_{14}$ \\ \hline
    $a_2$ & $h_{21}$ & $h_{22}$ & $ h_{23}$ & $h_{24}$ \\
    \hline
  \end{tabular}
\end{center}
Here, the row player is the attacker with $2$ attack actions. The column player is the defender with $4$ configurations. The reward/loss to the players are described by the matrix entries $h_{ij}, i \in \{1,2\}, j \in\{1, 2, 3, 4\},$ which are the rewards to the attacker when he uses $a_i$ to attack and the defender uses configures the system at $c_j$. The defender can relies on this model and assesses his best-effort worst-case security. The saddle-point equilibrium of this game yields a game value that quantifies the level of the security under the best-effort of the defender. It also leads an insight for the defender on how to choose a secure configuration to safeguard the system for a prescribed attack model. 


The analysis of the saddle-point equilibria of the security game has the following implications. First, the equilibrium strategies provide a security strategy for the defenders and protect the system in the worst-case scenario that is assumed by the defender. Such strategies are computed ahead of time. The operator can use them to maintain the connectivity of  the  {UAV} at each time $k$ robust to the worst-case adversarial behaviors within a range of attack behaviors. In many cases, the exact knowledge of the worst-case may not always be available. The overestimate of the capability of the attacker will result in a conservative solution while the underestimate will lead to a successful attacker and failure in the operation when the attack is not correctly anticipated. There is a need to consider strategies other than protections or preventions to safeguard the system. One type of strategy that can be built on top of the robust mechanism is the resiliency mechanism. In the case of the underestimate, the system is well prepared and designed to quickly recover from the attack. In the case of the overestimate, the resources used to strengthen the network for extremely low likelihood events can be used for the repair of the links and the restoration of the services. With limited resources, the defender needs to find an optimal tradeoff between the robustness and the resiliency to mitigate the impact of the attacks and maintain an acceptable level of system performance.  This joint robust and resilient mechanism has been studied in \citep{chen2019dynamic} and applied to multi-agent robotic systems in \citep{nugraha2019subgame,nugraha2020dynamic}.  %supplementary mechanisms to improve in these two circumstances.

Second, the value of the game obtained from the equilibrium analysis provides a predicted outcome and performance of the system. It provides a worst-case performance guarantee and a quantified assessment of the risks. In the example of  {UAV} networks, the solution to the zero-sum game from solving (\ref{maxminproblem}) provides a way for the designer to assess whether the network is still connected under the worst-case adversary. If it is, the designer can assess the security margin from being disconnected. Otherwise, the designer needs to find mechanisms other than  the control variable $u(k+c)$ to strengthen the network. For example, instead of using mobility to create connectivity, the designer can introduce additional communication resources, e.g., construction of ad hoc base stations, or the use of satellite communications. This design choice is another layer of optimal planning of resources since additional mechanisms are also constrained by limited resources.
In \cite{zhu2010network}, the authors see the value of games as the security capacity of a system. This is because when the computed value is below the targeted value, it means that it is impossible for the system to be secure for the given attack model unless additional resources are invested in the system. Games have also been studied for the overall design of secure communication layers as networks by \cite{rass_complexity_2014}.



%Another example of the game is the inspection games. One basic version of the inspection game involves two players. One is the inspector and the other one is inspectee. Inspector aims to select items or check points to verify and determine whether they are
%
%
%
%
%Inspection games
%
%The goal of

 \section{Multi-Stage and Multi-Phase Games}\label{msmp}


In Section \ref{gamemodels}, we have presented game theory as a tool to understand cybersecurity. In this section, we extend the game-theoretic technique developed for cyber attacks and connect it with the physical models of robots. The target of many  {APT} is to create malfunction of the physical assets, including a power plant, an autonomous vehicle, or a water treatment plant. By incorporating the physical models into the security game framework, we can provide a cross-layer security framework for robots and develop tailored cyber protection for the given robot systems that have specific operational system specifications and requirements.

To illustrate this concept, we use a generic nonlinear dynamical system in (\ref{dynamics}) to capture the mechanical behaviors of the robots. Let $x(t)$ be the state of the physical system and $y(t)$ be the output of the system. The physical dynamics of the robot systems, such as mechanical arms, walking robots,  {UAV}, can all be written into the following form:
 \begin{eqnarray}\label{dynamics}
 \dot{x}(t) &=& f(t, x, u; \theta(t, a, d)),\\
 y(t)&=& h(t, x, u; \theta(t, a, d)).
 \end{eqnarray}

Here, $f$ and $h$ are continuous functions in $(t, x, u)$. The physical system is controlled by the feedback law $u$ to achieve stabilization or targeted performances.
 $\theta(t, a, d)$ is the cyber state of the robot. It can represent the state  on the attack graph or the high-level description of the well-being of the cyber system. The state of the cyber system is influenced by the attack strategies $a$ and the defense strategies $d$. A well-designed defense can reduce the probability of the system in a compromised cyber state and allow the cyber system to recover quickly once it is attacked. From (\ref{dynamics}), it is clear that the cyber defense and attack not only directly affect the cyber state but also indirectly creates an impact on the physical system. For example, when the attacker gains access to the \ros nodes, he can modify the control logic and turn the robot into a deadly weapon \citep{clark2013impact,xu2018cross}. In the scenarios of multi-agent systems, one robot can be misled by a compromised robot to put the team into jeopardy and fail the mission \citep{xu2015cyber,Quanyan2013CCPS}.

 %  The cyber state may not be always directly observable and need to be constantly estimated over time.

 \begin{figure}[t]
    \centering
     \includegraphics[scale=0.5]{figures/3phase.png}
    \caption{Multi-stage and multi-phase interactions between an attacker and a defender: The attacker changes the cyber state $\theta$ to affect the physical state $x$ at the last stage of Phase $3$.} \label{3phase}
\end{figure}

The goal of the extended game framework is to capture this impact so that the defense designed at the cyber layer will reduce the cyber-physical risks and the control designed at the physical layer will be able to quickly mitigate the physical damages when an attacker succeeds at the cyber layer. To capture these multiple layers of effects, authors in \citep{zhu2018multi,huang2018gamesec,rass_gadapt:_2016} have created a multi-stage and multi-phase game model. The entire attack process is decomposed into multiple phases that represent multiple rounds or stages of interactions between the attacker and the system at different layers. At Phase 1, the attacker aims to create social engineering approaches to infect the system. To defense against this attack, defenders can raise security awareness, provide training to users and employees, or developing incident documentation and alert system to prevent malicious outsiders from entering the system or the insider to behave abnormally.

At Phase 2, the attacker aims to maximize the infection, search for its targeted asset and get closer to it. The defender at this phase can leverage spot-checking to detect virus/malware, change system configurations, or develop proactive defense mechanisms (e.g., honeypots \citep{jajodia2016cyber,mokube2007honeypots} and moving target defenses \citep{zhu2013game,jajodia2011moving}) to reduce the system risks. At Phase 3, the attacker aims to create physical damage on the system on the asset. It is already late for the defender to prevent the asset at this stage from damages. However, the defender can detect anomalous behaviors and reconfigure the control at the physical layer to reduce the impact of the attack and develop mechanisms to recover the system from the attacks.

The multi-stage multi-phase interactions are illustrated in Fig. \ref{3phase}. Each phase contains several stages of interactions. The success of an attacker in one phase will lead him to the next phase until he takes over the control of the physical assets. The state of the cyber system $\theta$ evolves over these multi-round interactions. In Phase 3, a compromised cyber state will influence the physical state $x$. The control taken at the end of Phase 3 can mitigate the physical impact of the attacker.

\begin{figure}[t]
\centering
     \includegraphics[scale=0.5]{figures/flipit.png}
    \caption{Illustration of FlipIt games: The attacker and the defender compete to control a shared resource. Both players can choose  when to move at any time. Each move incurs a cost. The player controls the resources for a period of time after his move till the next move of the other player.} \label{flipit}
\end{figure}

Each phase has unique attacker-defender interactions. They can be modeled using a suitable game-theoretic framework. In the first phase, the game often involves a human user and an attacker. The goal of the attacker is to use social engineering techniques to deceive the users to gain credentials for access. In \citep{van2013flipit}, FlipIt games have been proposed to understanding many cybersecurity scenarios. Consider the scenario where a user can choose when to change his passwords and an attacker can choose the time to hack the account. A weak password that has not been changed for a long time can be eventually leaked to the attacker. One way to protect a user's account to frequently change the password. However, it would create a perceived overhead if a user changes the password too frequently, and \cite{rass_password_2018} gives a game model to find an optimal tradeoff between security and usability here. From the attacker's perspective, there is a cost for him to gain reconnaissance and hack the account. FlipIt games capture the strategic decision of both players. The game analysis provides a risk assessment of the system and the development of defense strategies. The applications of FlipIt games have been extended to many applications including cloud computing \citep{pawlick2015flip,xu2015secure,chen2016optimal}, cybercrime \citep{canzani2018risk,basak2018initial}, and  {IoT} systems \citep{chen_optimal_2016,pawlick2018istrict}.

In the second phase, an intelligent attacker can move stealthily and strategically in the network to gain access to the targeted asset.  {APT} are this type of threat that is capable of customizing their strategies against specific targets and disguise themselves for a prolonged period. Once the  {APT} attackers enter the system, they escalate their privilege and propagate laterally in the network, compromising other nodes to gain deeper access to find their target. The goal of the defender is to detect the compromise nodes and respond quickly to prevent the attacker from going deeper and reaching critical assets. A game modeling this type of interactions is \textsc{Cut-The-Rope} (Section \ref{sec:cut-the-rope}), but other models have also been proposed, using sequential games \citep{huang2020dynamic,huang2019adaptive,noureddine2016game}. One important application of these models is to develop proactive defenses. They provide a precautious and strategic way to increase the cost of attack while mitigating the potential damage attacker could bring to the final target. An effective proactive response system can delay the attack and give network administrators a sufficient amount of time to meticulously analyze data and deploy effective responses to the threats.

In the third phase, an attacker has successfully gained access to the critical asset and aims to create maximum impact. The goal of the defender in this phase is to reduce the damages that can be created by the attacker. An example of games that capture this scenario is the Flip the Cloud game described in \citep{pawlick2015flip}. An  {APT} attacker can take hold of the cloud and sends falsified information to mislead a robot that relies on the computations in the cloud. The analysis of the game between the cloud that is taken over by the attacker and the system leads to a strategic trust mechanism \citep{pawlick2018istrict} that can filter and reject misleading information and an event-triggered control mechanism \citep{xu2015secure} to switching the control laws to maintain an acceptable level of performance. Here, the goal of physical control is to strengthen the resiliency of the robots. With a suitable design, the robots can still carry on their missions and complete their tasks despite the compromised cyber state and the unanticipated events. The resilient control problem has been discussed in \citep{zhu2011hierarchical,rieger2019,rieger2012agent}. Game-theoretic techniques to achieve resiliency of the control system performance have been studied in \citep{zhu2013resilient,huang2020dynamic,zhu2012dynamic,chen2019dynamic,
 RCSmetric}.

%\begin{remark}[on how to distinguish two kinds of  {APT}]
Generally, it is advisable to consider  {APT} models relative to what the adversary tries to accomplish in the long run, as \citep{rass_cyber-security_2020} distinguishes two types of  {APT}:
\begin{itemize}
	\item One type is about \emph{gaining long-run control} over the victim, but without ultimately destroying it. This can be the case when an industrial robotics-enhanced production line is hacked for the purpose of quality dropout increase, or to induce flaws in the products, up to inserting malicious parts or similar. Other scenarios include the overtake of an infrastructure of unintended purposes, e.g., cryptocurrency mining or similar. FlipIt is a class of game models to defend against this type of  {APT}.
	\item The other type aims at \emph{killing the victim}, which entails a slow and ubiquitous penetration staying beneath the detection radar so that it is too late for the defender to react when the attacker becomes visibly active. Examples of such incidents have been reported on large critical infrastructures, with Stuxnet being an early and famous example. Game models for this type of  {APT} are, among others, \textsc{Cut-The-Rope}.
\end{itemize}
%\end{remark}

  \subsection{Signaling Games for Multi-Phase Security}

In the security games across the three phases, the players often have incomplete information regarding the payoffs, action sets, and the type of opponents the players interact with. It is essential for security games to capture these uncertainties in the game. Signaling games are a common class of games that have been used to model the sequential interactions between two players under incomplete information. They have been used in many applications such as cyber deception \citep{pawlickgame,pawlick2018modeling,zhuang2010modeling,pawlick2019game,pawlick2015deception}, communication networks \citep{rahman2013game,carroll2011game}, and trust management \citep{casey_compliance_2016,moghaddam2015trust,pawlick2017strategic}. In this class of games, one player is the sender, denoted by $S$, and the other player is the receiver, denoted by $D$. The sender has private information $\theta \in \Theta$ unknown to the receiver and sends a signal\footnote{The literature also uses the term ``message'' in the context of signalling games, which we avoid here to prevent ambiguities with the term ``message'' as data in transit like in Chapter \ref{sec:cyber-issues-et-al}.} $m \in \mathcal{M}$ to the receiver. The goal of the receiver observes the signal $m$ and chooses an action $a \in\mathcal{A}$ to respond to the signal so that his reward $U_S(\theta, m, a)$ is maximized. The goal of the sender is to pick a signal that will lead to a desirable action chosen by the receiver so that his reward $U_R(\theta, m, a)$ is maximized. Both players have the knowledge of how this game is played. More specifically, the players know the reward functions and action sets of both players. The private information $\theta$ is modeled as a random variable. Both players have knowledge of the distribution of the random variable. However, only the sender knows the realization of $\theta$.

 This game is illustrated by an extensive-form game in Fig. \ref{signaling}. Nature first chooses $\theta$ according to the distribution known to the players. The sender who observes $\theta_1$ or $\theta_2$ will pick a signal $m\in\{m_1, m_2\}$. The receiver cannot distinguish between the type of the players (indicated in the figure by the information set of the receiver) but can only choose an action $\{a_1, a_2\}$ based on his observation of the signal.  The strategies of the players are described by the policies $\mu_S: \Theta\rightarrow \mathcal{M}$ and $\mu_R: \mathcal{M}\rightarrow \mathcal{A}$ that are determined prior to the start of the game. The players use the policies to determine their actions based on their private observations.  Bayesian perfect Nash equilibrium is commonly used as the solution concept for the signaling games. An equilibrium profile $(\mu^*_S, \mu^*_R )$ is  a Bayesian perfect Nash equilibrium if it satisfies sequential rationality and there exists a consistent belief system, a distribution over the information set, that supports this equilibrium profile. Readers can refer to the mathematical details in \citep{gibbons1992game} for the analysis and the computation of the equilibrium.

%change of measure in signaling games.

 \begin{figure}[t]
    \centering
     \includegraphics[scale=0.5]{figures/signaling.png}
    \caption{Signaling games between one sender and one receiver. The sender has private information $\theta$ and sends a signal $m \in \mathcal{M}=\{m_1, m_2\}$ to the receiver to achieve an outcome that optimizes his reward. The receiver determines action $a \in \mathcal{A}=\{a_1, a_2\}$ to maximize his reward. The dotted line indicates an information set of player 2. } \label{signaling}
\end{figure}

Signaling games can be used to capture information asymmetry, where one player has more information than the other player. It is a pervasive phenomenon in cybersecurity. Across the three phases depicted in Fig. \ref{3phase}, the system defender may not distinguish the attacker from the normal users. In contrast, the attacker can observe the behaviors of the system. In \citep{pawlick_phishing_2017}, signaling games have been used to model phishing. An attacker sends a phishing email to a population of receivers while a user relies on spam and scam detection systems to filter out a suspicious email from the primary inbox.



 An extension of the signaling games to multiple rounds of interactions has been studied in \citep{farhang2014dynamic,huang2020dynamic}. The multi-round game models are used to study the Phase 2 interaction where the attacker aims to escalate his privilege and gain access to the targeted asset.
 In \citep{xu2015cyber}, a trust mechanism based on signaling games has been developed for  {UAV} at Phase 3 as the last shield to defend against the attacker. Once an attacker has an access to the remote control station, he can send a falsified control command to direct the  {UAV} to hit a building. The trust mechanism enables the  {UAV} to make onboard decisions of following or rejecting the command when they predict that following the command would lead to catastrophic consequences. 
%an evolutionary game has been proposed to study the ins the phishing games in phase 1 has been studied in \cite{}. Phase 2 is the attacker of the ... it is been studied in  \cite{insider threat}. {flipit games}

 \begin{figure}[t]
    \centering
     \includegraphics[scale=0.7]{figures/nestedgames.png}
    \caption{G$1$, G$2$, and G$3$ represent games at three phases. The three games are nested. The outcome of the game at earlier phases will affect the structure of the game in the later phases. The defense strategies need to be planned backward from the last phase.} \label{nestedgames}
\end{figure}

  \subsection{Games-in-Games Model}\label{gigm}

The games in the three phases are interdependent. The actions chosen by the defender and the attacker in the first phase will affect the cyber state and the structure of the game played in the second phase. When planning the defense at the first phase, it is essential to understand its consequences on the following phases and make an effective planning decision at the first phase. The games at the three phases can be integrated into a game-in-games \citep{huang2020dynamic,zhu2015game,xu2016cross,chen-TCNS-19-games,nugraha2019subgame,xu2018cross,xu2017game}, in which the game at an earlier phase is nested in the game at a later phase.  Illustrated in Fig. \ref{nestedgames}, the game-of-games integration gives a holistic view of the security issues across multiple layers of robotic systems and provides a cross-layer risk assessment and design methodology of security mechanisms. 

Security games for sophisticated attacks often require an integrated model that composes interactions at different layers, stages, or phases of the system. The game-in-games leverage the sequential nature of the cyber attacks and provide a framework to compose local-stage games into an integrated large-scale game for a holistic analysis of the risks. The computation of the equilibrium solutions at each phase is backward. The defense strategies in Phase 1 depends on the defense strategies in Phase 2, which is determined by the strategies in Phase 3. This backward computation will guarantee that the defense strategies are strategically optimal across the phases rather than myopically optimal within one single stage. Readers can refer to the recent book \citep{zhucross} for a comprehensive introduction of the game-theoretic techniques for cross-layer designs. 

\input{subsections/control}

\section{Examples of Game-Theoretic Analysis}
We provide two case studies to elaborate on the application of game theory to robot security. The first one introduces the application of signal games to  {UAV} and develops a cyber-physical trust interface between the  {IT}-level signals and the  {OT}-level operations and controls. The second one continues the example described in Fig. \ref{uav} and discusses how to design control mechanisms that can fend off jamming attacks while maintaining connectivity.

\subsection{Signaling Games and  {UAV}}


This case study presents a team of multi-agent  {UAV} with $n$ autonomous agents (ASs) and a control station (CS). Each agent has two components. One is the physical layer  which implements real-time control to achieve its control objectives. The other one is the cyber layer which sends information and signals to the agents as inputs for the controller. At the physical layer, a min-max model predictive control (MPC) problem is formulated to handle the worst-case disturbances based on the model. For AS agent $i$ at time $k$, the problem is formulated as a zero-sum game between the controller and the disturbance:
\begin{align}
    \mathcal{P}_k^i:  \min_{\hat{u}^i_k}\max_{\hat{w}^i_k} \ \ \ J_c\left(x_k^i,r_k^i,\hat{u}^i_k,\hat{w}^i_k\right).
\end{align}
Here, $J_c$ is the accumulated stage cost until horizon-window $N$; $x_k^i$ is the state vector; $r_k^i$ is the reference trajectory given by the CS; $\hat{u}^i_k$ and $\hat{w}^i_k$ are the estimated control and disturbance vectors. An adversary can fabricate a fake reference signal $r^i$ to deviate agent $i$ from its real
trajectory to achieve Suicidal Attack (SA) or Collision
Attack (CA).

At the cyber layer of ASs, we use a signaling game method to capture the information asymmetry and multi-stage behaviors of these players. The CS (sender $S$) has a binary private type $\theta$ denotes whether $S$ is normal or malicious. $S$ sends a signal $r^i$ to each AS (receiver $R^i$). Before choosing action $a^i$, AS updates its beliefs about the type $\theta$ using Bayes' rule and prior belief $p^i(\theta)$. The goal of $R^i$ is to choose an action $a^i$ to minimize its expected cost $c_R^i$ given a posterior belief $\mu^i(\theta|r^i)$, while the goal of the sender is to choose a signal $r^i$ to minimize the cost $c_S$ by anticipating the behavior of the receiver $R^i$. The game admits a  {PBNE}, which is a strategy profile $\{\sigma(S),\sigma_R^i\}$ and posterior beliefs $\mu^i(\theta|r^i)$ such that
\begin{align}
    &\forall \theta, \quad \sigma_R^i(r^i)\in\arg\min_{a^i} \sum_{\theta}\mu^i(\theta|r^i)c_R^i(r^i,a^i,\theta),\\
    &\forall\theta, \quad 
    \mathbf{\sigma}_S(\theta)\in\arg\min_{\mathbf{r}} c_S(\mathbf{r},\mathbf{\sigma}_R,\theta)
\end{align}
where posterior beliefs $\mu^i(\theta|r^i)$ are updated according to Bayes' rule. There are two  {PBNE} that exist in this cyber-physical signaling game. One is a separating equilibrium, and the other is a pooling equilibrium. Both  equilibria can lead to the protection of ASs from collisions as the equilibria can guarantee that $R^i$ only accepts reference trajectory $r^i$ if it is out of the danger zones. The designed framework yields an intelligent control of each agent to avoid collisions.  Illustrated in Fig. \ref{uav}, a group of  {UAV} reject the falsified command and switch the system to a safe control mode. The  {UAV} hover in the air and keep a safe distance from each other and the building.  The results indicate that the integrative framework enables the co-design of cyber-physical systems to minimize the damages, leading to online updating the cyber defense and physical layer control decisions. Interested readers can refer to \cite{xu2015cyber} for more details on this case study.

 \begin{figure}[t]
\centering
     \includegraphics[scale=0.5]{figures/uav.png}
    \caption{Trust mechanism implemented in the  {UAV} control system. The  {UAV} start to hover before they hit the building.} \label{uav}
\end{figure}



\subsection{Jamming Games and Multi-Agent Systems}

Multi-agent systems provide a framework for studying distributed decision-making problems as a number of agents make local decisions by interacting with each other over networks. One of the common security threats in networked systems is jamming attacks. The adversary can simply transmit interference signals to interrupt communication among agents. Non-cooperative game theory approaches can be used to find the optimal defense mechanism to prevent and restore the network from successful attacks. %the optimal attacker-defender behaviors are widely used for addressing security problems including jamming attack. However, in previous studies, optimal strategies for the attackers have not been well addressed and no defense mechanism is developed to mitigate the attacks and restore the communication.

We model the interaction between an attacker
and a defender in a two-player two-stage game setting. The attacker is motivated to disrupt the communication by attacking individual links. The attack model consists of a jammer who chooses the links and the durations of the attack with the knowledge of the communication graph of the  {UAV} and the energy constraints. The defender can recover a subset of links that are important for maintaining the connectivity of the graph with limited energy. %Fig. 1 illustrates the timeline of the attack and the recovery sequences.

In the game, both players attempt to choose the best strategies to maximize their own utility functions. The utilities for the attacker $U^A$ and the defender $U^D$ are defined as the total generalized edge connectivity (with the negative sign for the attacker), plus the cost for jamming (attacker) or recovering (defender). The two-stage game is played as follows. The jammer first attacks and then the defender recovers in the subgame. Let $m^A$ be the attacked edges and $\sigma^A$ be the attack intervals; let $m^D$ be the edges recovered and $\sigma^D$ be the recovery intervals. The strategies of the attacker and the defender are in terms of $(m^A, \delta^A)$ and $(m^D, \delta^D)$, respectively. 

The subgame perfect Nash equilibria are obtained using backward induction. Given the attacker's strategy $(m^A, \delta^A)$, the defender decides the best response strategy as
\begin{align}
    \left(m^{D*}(m^A,\delta^A),\delta^{D*}(m^A,\delta^A)\right)
    \in \arg \max_{(m^D, \delta^D)}U^D((m^A, \delta^A),(m^D, \delta^D))
\end{align}
Likewise, given the initial network graph $\mathcal{G}$, the attacker decides the strategy as
\begin{align}
    \left(m^{A*},\delta^{A*}\right)  \in \arg \max_{(m^A, \delta^A)} U^D((m^A, \delta^A),\left(m^{D*}(m^A,\delta^A),\delta^{D*}(m^A,\delta^A)\right))
\end{align}

This game can be applied to a multi-agent consensus problem, where the game is played repeatedly over time. In such a case, the energy constraints are extended to satisfy continuous communications. Fig. \ref{jammingresult} shows the states of the agents and properties of the players, with the agents achieving approximate consensus at  $t \approx 4$ with tolerance $\epsilon = 0.5$. This framework enables the study of how the attacks and recovery strategies affect the consensus process of the multi-agent systems. By analyzing the games, we can find the optimal strategies for the attacker and the defender in terms of edge connectivity and the number of connected components of the graph. Interested readers can refer to \cite{nugraha2020dynamic} for more details on this case study.

%We compare the results with different energy parameters.  Experimental result indicates that the attacker with more energy will attack all edges to make the recovery time of the defender shorter. Next, we compare the strategies of the players under path graph and complete graph. For the complete graph the attacker chooses to attack for shorter duration compared to the attacks in the path graph due to the high connectivity of the graph structure. Besides, we also show that different energy and cost will also influence the optimal strategy selection. 

 \begin{figure}[t]
\centering
     \includegraphics[scale=0.8]{figures/jammingresult.png}
    \caption{The state trajectories of the  {UAV}. The green areas indicate the intervals where the defender recovers. The red areas indicate
the intervals where the attacker attacks. The four agents reach consensus after $t \approx 4$ \cite{nugraha2020dynamic}. } \label{jammingresult}
\end{figure}
 



